Foliations of asymptotically flat manifolds by surfaces of Willmore type

The goal of this paper is to establish the existence of a foliation of the asymptotic region of an asymptotically flat manifold with nonzero mass by surfaces which are critical points of the Willmore functional subject to an area constraint. Equivalently these surfaces are critical points of the Geroch-Hawking mass. Thus our result has applications in the theory of General Relativity.

==> apriori3.tex <==
\section{Position estimates II}
\label{sec:position-estimates II}
Here we show how to estimate various terms appearing in the position estimate of the previous chapter. We assume
\begin{itemize}
\item[1)] $H\le \frac{c}{R}$ (perhaps we even don`t need this) and
\item[2)] $R\le c r_{\operatorname{min}}$.
\end{itemize}

The following lemma is not needed in the sequel, but we include it
since we might need it later.

\begin{lemma}\label{linfinityestimates}
For every solution of \eqref{eq:1} we have
\begin{align}
\rmin||\nabla H||_{L^\infty(\Sigma)}+||\Acirc||_{L^\infty(\Sigma)}\le C\rmin^{-2-\varepsilon}\label{linf1}
\end{align}
\end{lemma}
\begin{proof}
Using \eqref{eq:7} we estimate
\begin{align*}
||\Delta \Acirc||_{L^2} \le& c(||\nabla^2 H||_{L^2}+||H||_{L^\infty}||\Acirc||_{L^4}^2+||H||_{L^\infty}^2||\Acirc||_{L^2}+||\Acirc||_{L^6}^3\\
&+|| \RiemM||_{L^\infty}||\Acirc||_{L^2}+||\nabla \omega||_{L^2})\\
\le& \frac{c}{R^3},
\end{align*}
where we used Theorem \ref{thm:curv-est-1}, Corollary \ref{thm:A0-l2-1}, \eqref{eq:12} and Definition \ref{def:asymptotically-flat}. Using an integration by parts argument as in the proof of Lemma \ref{thm:estimate_d2H} we get
\begin{align*}
||\nabla^2 \Acirc||_{L^2} \le \frac{c}{R^3}.
\end{align*}
Hence we can apply Lemma $2.8$ of \cite{Kuwert-Schatzle:2001} (check that this is also true for embeddings in asymptotically flat manifolds!!!) and get
\begin{align*}
||\Acirc||_{L^\infty}^4 &\le c||\Acirc||_{L^2}^2(||\nabla^2 \Acirc||_{L^2}^2+ ||H||_{L^\infty}^4||\Acirc||_{L^2}^2)\\
&\le \frac{c}{R^8},
\end{align*}
where we used the above estimate for $\nabla^2 \Acirc$ and Corollary \ref{thm:A0-l2-1}. This proves the $L^\infty$-estimate for $\Acirc$. For the estimate of $\nabla H$ we differentiate \eqref{eq:1} and get
\begin{align*}
||\nabla \Delta H||_{L^2}\le& c(\lambda ||\nabla H||_{L^2}+ ||\Acirc||_{L^\infty}^2||\nabla H||_{L^2}+||H||_{L^\infty}||\Acirc||_{L^\infty}||\nabla \Acirc||_{L^2}\\
&+||\operatorname{Ric}||_{L^\infty}||\nabla H||_{L^2}+||H||_{L^\infty}||\nabla \operatorname{Ric}||_{L^2})\\
\le&\frac{c}{R^4}.
\end{align*}
Hence
\begin{align*}
||\nabla^3 H||_{L^2}\le \frac{c}{R^4}.
\end{align*}
Arguing as above we get
\begin{align*}
||\nabla H||_{L^\infty}^4&\le c||\nabla H||_{L^2}^2(||\nabla^3 H||_{L^2}^2+\frac{c}{R^4}||\nabla H||_{L^2}^2)\\
&\le \frac{c}{R^{12}}.
\end{align*}
This finishes the proof of the Lemma. 
\end{proof}
\begin{lemma}\label{acirc}
Let $F:(-\varepsilon,\varepsilon)\times \Sigma \rightarrow M$ be a family of embeddings with $\frac{d}{ds}F|_{s=0}=f\cdot \nu$. Then we have
\begin{equation}\label{acirc1}\begin{split}
 \frac{d}{ds}\Big|_{s=0} \int_\Sigma |\Acirc|^2 d\mu =&\ 2\int_\Sigma
 \Big(\nabla^j f \nabla_i \Acirc^i_j
 -f(\operatorname{tr}(\Acirc)^3+\frac{H}{2}|\Acirc|^2\\
&\ \qquad -\Acirc^i_j \text{{\it Riem}}_{0\ 0\, i}^{\ j})\big)\, d\mu\ . 
\end{split}\end{equation}
\end{lemma}
\begin{proof}
This directly follows from the well-known evolution equations for the various geometric quantities (see e.g. Huisken and Polden [???]).
\end{proof} 
\begin{lemma}\label{div}
Let $F:(-\varepsilon,\varepsilon)\times \Sigma \rightarrow M$ be a family of embeddings with $\frac{d}{ds}F|_{s=0}=f\cdot \nu$. Then we have
\begin{align}
 \frac{d}{ds}|_{s=0} \int_\Sigma (Ric(\nu,\nu)-\frac{Sc}{2})d\mu=\int_\Sigma (G^i_jh^j_i f-Ric(\nabla^\Sigma f,\nu)) d\mu, \label{div1}
\end{align}
where $G=Ric-\frac{Sc}{2}id$ is the Einstein tensor.
\end{lemma}
\begin{proof}
First of all we calculate
\begin{equation}\label{div2}\begin{split}
 \frac{d}{ds}|_{s=0} \int_\Sigma (Ric(\nu,\nu)-\frac{Sc}{2})d\mu=&\int_\Sigma \Big(f\nabla^M_\nu Ric(\nu,\nu)-2Ric(\nabla^\Sigma f,\nu) \\
&-\frac{f}{2}\nabla^M_\nu Sc +(Ric(\nu,\nu)-\frac{Sc}{2})Hf\Big)\, d\mu.
\end{split}\end{equation}
We also know that $G$ is divergence-free and therefore for an
orthonormal basis $e_0,e_1,e_2$,
\begin{align*}
0=\operatorname{div}(G)(v)=\sum_{i=0}^2 g(\nabla_{e_i}(G(v))-G(\nabla_{e_i} v),e_i).
\end{align*}
Let now $X$ be given by $X=G(\nu)=Ric^i_j \nu^j -\frac{Sc}{2} \nu^i$, then we have
\begin{align}
\operatorname{div}_M (X)=\sum_i g(\nabla_{e_i} X,e_i)=\sum_i g(G(\nabla_{e_i} \nu),e_i).\label{div3}
\end{align}
Moreover we have (by taking $e_0=\nu$ and $e_1,e_2$ tangent to $\Sigma$)
\begin{align}
\operatorname{div}_M(X)&=\operatorname{div}_\Sigma (X)+g(\nabla^\Sigma_\nu X,\nu) \nonumber \\
&=\operatorname{div}_\Sigma (X)+g(\nabla_\nu(G(\nu)),\nu). \label{div4}
\end{align}
Next we compute using the first variation formula
\begin{align}
\int_\Sigma (Ric(\nu,\nu)-\frac{Sc}{2})Hfd\mu =&\int_\Sigma g(fX,H\nu)d\mu \nonumber \\
=& \int_\Sigma \operatorname{div}_\Sigma (fX)d\mu \nonumber \\
=& \int_{\Sigma} (f\operatorname{div}_\Sigma (X)+g(\nabla^\Sigma f,X))d\mu \nonumber \\
=& \int_\Sigma (f\operatorname{div}_M (X)+g(\nabla^\Sigma f,X)\nonumber \\
&-fg(\nabla_\nu (G(\nu)),\nu))d\mu \label{div5}.
\end{align}
Now we calculate
\begin{align*}
\nabla_\nu(G(\nu))=& (\nabla_\nu G)(\nu)+G(\nabla_\nu \nu)\\
=& (\nabla_\nu Ric)(\nu)- \frac{\nabla_\nu Sc}{2} \nu-\frac{1}{f}G(\nabla^\Sigma f)
\end{align*}
and therefore
\begin{align}
fg(\nabla_\nu (G(\nu)),\nu)=f\nabla_\nu Ric(\nu,\nu)-\frac{f}{2} \nabla_\nu Sc-Ric(\nabla^\Sigma f,\nu).\label{div6}
\end{align}
Next we get from \eqref{div3} 
\begin{align}
\operatorname{div}_M(X)=& \sum_{k=0}^2 g(G(\nabla_{e_k} \nu),e_k)\nonumber \\
=& \sum_{i,j=1}^2 g(G(h_i^j e_j ),e_i)+g(G(\nabla_\nu \nu),\nu)\nonumber \\
=& \sum_{i,j=1}^2g(G(h_i^j e_j ),e_i)-\frac{1}{f} g(G(\nabla^\Sigma f),\nu)\nonumber \\
=& \sum_{i,j=1}^2g(G(h_i^j e_j ),e_i)-\frac{1}{f} Ric(\nabla^\Sigma f,\nu). \label{div7}
\end{align}
Inserting \eqref{div6} and \eqref{div7} into \eqref{div5} gives
\begin{align}
\int_\Sigma (Ric(\nu,\nu)-\frac{Sc}{2})Hfd\mu=& \int_\Sigma (f g(G(h_i^j e_j),e_i)-Ric(\nabla^\Sigma f,\nu) +g(\nabla^\Sigma f,X)\nonumber \\
&-f\nabla_\nu Ric(\nu,\nu)+\frac{f}{2}\nabla_\nu Sc+Ric(\nabla^\Sigma f,\nu))d\mu \nonumber \\
=&\int_\Sigma (f g(G(h_i^j e_j),e_i)+Ric(\nabla^\Sigma f,\nu) \nonumber \\
&-f\nabla_\nu Ric(\nu,\nu)+\frac{f}{2}\nabla_\nu Sc)d\mu, \label{div8}
\end{align}
where we used that
\begin{align*}
g(\nabla^\Sigma f,X)=g(\nabla^\Sigma f,G(\nu))=Ric(\nabla^\Sigma f,\nu).
\end{align*}
Combining \eqref{div2} and \eqref{div8} finishes the proof of the Lemma.
\end{proof}
\begin{theorem}\label{position}
Irgendwelche guten Voraussetzungen. We have
\begin{align}
\frac{|a|}{R}= o(1).\label{position1}
\end{align}
\end{theorem}
\begin{proof}
From \eqref{eq:14} and Gauss-Bonnet we know that
\begin{align*}
8 \pi \chi (\Sigma) =\int_\Sigma(H^2 -|\Acirc|^2 -4(Ric(\nu,\nu)-\frac{Sc}{2}))d\mu
\end{align*}
and hence
\begin{align}
0=\frac{d}{ds}\Big|_{s=0}\int_\Sigma(H^2 -|\Acirc|^2 -4(Ric(\nu,\nu)-\frac{Sc}{2}))d\mu. \label{position2}
\end{align}
Now we calculate term by term. Since we study critical points of the Willmore functional under an area constraint we know that
\begin{align}
\frac{d}{ds} \Big|_{s=0}\int_\Sigma H^2d\mu =& -\lambda \int_\Sigma \xi H d\mu \nonumber\\
=&\ O(R^{-3}), \label{position3}
\end{align}
where we used Propsosition \ref{lambda} and the estimate for $\int_\Sigma \xi H d\mu$ from \cite{Huisken-Yau:1996}. Next, from Lemma \ref{acirc} with $f=\xi$ we know that
\begin{align*}
\Big| \frac{d}{ds} \Big|_{s=0}\int_\Sigma |\Acirc|^2 d\mu\Big| \le& 2 \Big|\int_\Sigma \nabla^j \xi \nabla_i \Acirc^i_jd\mu \Big|+c\int_\Sigma (|\Acirc|^3+H|\Acirc|^2 +|\Acirc| |Riem|)d\mu \\
\le& 2\Big| \int_\Sigma \nabla^j \xi \nabla_i \Acirc^i_jd\mu\Big|+ O(R^{-3}),   
\end{align*}
where we used the various estimates for $\Acirc$, $H$ and $Riem$. Moreover we use \eqref{babl}  and the fact that $|\nabla b|\le \frac{c}{R^2}$ to calculate
\begin{align*}
|\int_\Sigma \nabla^j \xi \nabla_i \Acirc^i_jd\mu| =& |\int_\Sigma \nabla_i \Acirc^i_j (\langle \nabla^j b, \nu \rangle + \Acirc^j(b^T)+\frac{H(b^T)^j}{2})d\mu |\\
\le& c\int_\Sigma |\nabla \Acirc|(|\nabla b|+|\Acirc|)d\mu\\
&+ |\int_\Sigma \Acirc^i_j\frac{ (b^T)^j \nabla_i H+H\nabla_i (b^T)^j}{2}d\mu| \\
\le& O(R^{-3})+\frac{1}{2}|\int_\Sigma \Acirc^i_j H \nabla_i (b^T)^j d\mu|.
\end{align*}
We have
\begin{align*}
\nabla_i (b^T)^j = \big(\nabla^\Sigma_i b^T\big)^j= \big(\Pi^T\nabla_i^M(b-\langle b,
\nu\rangle\nu)\big)^j =  \big(\Pi^T\nabla_i^M b\big)^j-\langle
b,\nu\rangle A_i^j 
\end{align*}
Using again that $|\nabla b|\le \frac{c}{R^2}$ and that $\Acirc^i_j A_i^j =|\Acirc|^2$ we estimate
\begin{align*}
|\int_\Sigma \nabla^j \xi \nabla_i \Acirc^i_jd\mu|\le O(R^{-3})
\end{align*}
%Using the properties of our asymptotically flat manifold (for example $|H-H^S|\le \frac{c}{R^2}$, ...) it is easy to see that
%\begin{align*}
%\int_\Sigma \Acirc^i_j H \langle b,\nabla_i \nu \rangle \nu^j d\mu =& \int_\Sigma (\Acirc^S)^i_j H^S g^S( b, \nabla^S_i \nu^s \rangle (\nu^S)^j d\mu^S +O(R^{-3}).
%\end{align*}
%On the other hand we know from the conformal invariance of $\int_\Sigma |\Acirc^S|^2 d\mu^s$ that
%\begin{align*}
%0=\frac{d}{ds}|_{s=0} \int |\Acirc^S|^2 d\mu.
%\end{align*}
%Repeating the above computations in the Schwarzschild case then yields
%\begin{align*}
%0=O(R^{-3})+|\int_\Sigma (\Acirc^S)^i_j H^S g^S( b, \nabla^S_i \nu^s \rangle (\nu^S)^j d\mu^S|.
%\end{align*}
Combining the estimates gives 
\begin{align}
 \frac{d}{ds} |_{s=0}\int_\Sigma |\Acirc|^2 d\mu=O(R^{-3}). \label{position4}
\end{align}
Finally we use Lemma \ref{div} with $f=\xi$ to get
\begin{align}
\frac{d}{ds}|_{s=0} \int_\Sigma (Ric(\nu,\nu)-\frac{Sc}{2})d\mu=&\int_\Sigma (G^i_jh^j_i \xi-Ric(\nabla^\Sigma \xi,\nu)) d\mu \nonumber \\
=& \int_\Sigma (\xi G^i_j\Acirc^j_i +\xi \frac{H}{2}(Ric_\alpha^\beta-\frac{Sc}{2}\delta_\alpha^\beta)(\delta_\alpha^\beta-\nu_\alpha \nu^\beta)\nonumber \\
&-Ric(\nabla \xi,\nu))d\mu \nonumber \\
=& O(R^{-3})-\int_\Sigma (\frac{H}{2}\xi Ric(\nu,\nu)+Ric(\nabla \xi,\nu))d\mu, \label{position5}
\end{align}
where we used that $h^j_i=\Acirc^j_i +\frac{H}{2}\delta^j_i$, $|G|\le cR^{-3}$, Lemma \ref{linfinityestimates} and the summation over $\alpha,\beta$ is from $0$ to $2$. Next we use \eqref{babl} to get
\begin{align*}
 \int_\Sigma (\frac{H}{2}\xi Ric(\nu,\nu)+Ric(\nabla \xi,\nu))d\mu=& \int_\Sigma \frac{H}{2} (Ric(b^N,\nu)+Ric(b^T,\nu))d\mu\\
 &+O(R^{-3})\\
=& \int_\Sigma \frac{H}{2} Ric(b,\nu)d\mu +O(R^{-3}).
\end{align*}
Combining this with \eqref{position3}-\eqref{position5} we get
\begin{align}
\int_\Sigma \frac{H}{2} Ric(b,\nu)d\mu=O(R^{-3}). \label{position6}
\end{align}
Moreover we can apply Theorem \ref{thm:umbilical} to get that
\begin{align*}
|\int_\Sigma (\frac{H}{2}-\frac{1}{R}) Ric(b,\nu)d\mu| \le& c||H-\frac{2}{R}||_{L^2(\Sigma)}||Ric||_{L^2(\Sigma)}\\
\le& c\frac{1}{R} \frac{1}{R^2}=O(R^{-3}).
\end{align*}
Hence it remains to calculate $\int_\Sigma Ric(b,\nu)d\mu$. We will do this here for $\Sigma=S_R(a)$, $Ric=Ric^S$ and $\nu=N$ since it is easily seen (to be worked out in detail) that the resulting errors in the genral case are of acceptable order.
Now we have with $\rho=r^{-1}(RN+|a|b)$
\begin{align}
\int_{S_R(a)} Ric^S(b,N) d\mu =& \int_{S_R(a)} \frac{m}{r^3} (g^e(b,N)-3g^e(\rho,N)g^e(\rho,b))dx+O(R^{-2})\nonumber \\
=& m\int_{S_R(a)} (\frac{g^e(b,N)}{r^3}-\frac{3}{r^3}(\frac{R^2}{r^2}g^e(b,N)+\frac{R|a|}{r^2}\nonumber \\
&+\frac{|a|R}{r^2}g^e(b,N)^2 +\frac{|a|^2}{r^2}g^e(b,N)))d\mu +O(R^{-2}) \label{position7}
\end{align}
Now we calculate these integrals using the formula of the previous chapter.
\begin{align*}
\int_{S_R(a)} \frac{g^e(b,N)}{r^3}d\mu =& -4\pi \frac{|a|}{R^2-|a|^2},\\
-3R^2\int_{S_R(a)} \frac{g^e(b,N)}{r^5}d\mu =& 4\pi R^2 \frac{|a|(5R^2-|a|^2)}{(R-|a|)^3(R+|a|)^3},\\
-3R|a|\int_{S_R(a)} \frac{1}{r^5}d\mu =& 2\pi R^2 (\frac{1}{(R+|a|)^3}-\frac{1}{(R-|a|)^3}),\\
-3R|a| \int_{S_R(a)} \frac{g^e(b,N)^2}{r^5}d\mu =& -4\pi |a| \frac{R^4+5R^2|a|^2 -|a|^4}{(R-|a|)^3(R+|a|)^3}\ \ \ \text{and} \\
-3|a|^2\int_{S_R(a)} \frac{g^e(b,N)}{r^5}d\mu =& 4\pi |a|^2 \frac{|a|(5R^2-|a|^2)}{(R-|a|)^3(R+|a|)^3}.
\end{align*}
Inserting this into maple we get
\begin{align}
\int_{S_R(a)} Ric^S(b,N) d\mu = 4\pi m \frac{|a|^5}{(|a|^2-R^2)^3}. \label{position8}
\end{align}
Assuming now that $|a|\le R$ (This actually should already follow from
the estimate, since otherwise the right hand side blows up - if we
know it initially) we combine these results to get
\begin{align}
\frac{c}{R} \ge& R\, \Big|\int_{S_R(a)}  Ric^S(b,N) d\mu\Big| \nonumber \\
=&\ \frac{4 \pi m R |a|^5}{ (R+|a|)^3(R-|a|)^3}\nonumber \\
\ge&\ \frac{\pi m|a|^5}{2 R^5}.\label{position9}
\end{align}
This finally implies that 
\begin{align}
\frac{|a|}{R} \le \frac{c}{R^{\frac{1}{5}}} \label{position10}
\end{align}
and finishes the proof of the Theorem.
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "master"
%%% End

==> apriori_alt.tex <==
\section{Integral curvature estimates}
In this section we will deriva a priori bounds on the curvature of
surfaces which satisfy the equation
\begin{equation}
  \label{eq:1}
  -2\Delta H - 2 H |\Acirc|^2 - 2 \Ric(\nu,\nu) = \lambda H
\end{equation}
where $\lambda$ is a constant. We will later make the assumption that
both $H>0$ and $\lambda >0$. Without the assumption on $\lambda$ we
can derive the following lemma.
\begin{lemma}
  \label{thm:init-integral}
  If $\Sigma$ satisfies equation~\eqref{eq:1} with  $H>0$, then
  \begin{equation*}
    \lambda |\Sigma|
    +
    \int_\Sigma 2 |\nabla \log H|^2 +
    \half H^2  + |\Acirc|^2\dmu
    \leq
    8\pi - \int_\Sigma \ScalM \dmu.
  \end{equation*}
  If $\lambda>0$ and $\ScalM\geq 0$ we find that
  \begin{equation*}
    2 \lambda |\Sigma|
    +
    \int_\Sigma H^2 \dmu \leq 16\pi
  \end{equation*}
\end{lemma}
\begin{proof}
  Multiply equation~\eqref{eq:1} by $H^{-1}$, and integrate the first
  term by parts. This yields
  \begin{equation}
    \label{eq:2}
    \lambda|\Sigma| + \int_\Sigma 2 |\nabla \log H|^2 + 2|\Acirc|^2 +
    2 \Ric(\nu,\nu)\dmu = 0.
  \end{equation}
  We can now use the Gauss equation~(\ref{eq:4}) to replace
  \begin{equation*}
     2\Ric(\nu,\nu) = \ScalM - \ScalSig + \half H^2 - |\Acirc|^2
  \end{equation*}
  substituting into~\eqref{eq:2} yields in view of the Gauss-Bonnet formula
  \begin{equation*}
    \lambda |\Sigma| + \int_\Sigma 2 |\nabla \log H|^2 +
    \half H^2  + |\Acirc|^2\dmu
    \leq
    8\pi - \int_\Sigma \ScalM \dmu.
  \end{equation*}
\end{proof}
This estimate already implies that the Hawking mass
\begin{equation*}
  m_H(\Sigma) = \frac{|\Sigma|^{1/2}}{(16\pi)^{3/2}} \left(16\pi
    -\int_\Sigma H^2\dmu\right)
\end{equation*}
is well behaved on such surfaces.
\begin{theorem}
  If $(M,g)$ satisfies $\ScalM\geq 0$ and if $\Sigma$ is a compact
  surface satisfying equation~\eqref{eq:1} with $H>0$ and $\lambda>0$,
  then $m_H(\Sigma)\geq 0$.

  Furthermore if $F : \Sigma\times[0,\eps) \to M$ is a variation with
  initial velocity $\ddeval{F}{s}{s=0} = \alpha\nu$ and $\int_\Sigma
  \alpha H \dmu \geq 0$, then
  \begin{equation*}
    \DD{}{s} m_H\big(F(\Sigma,s)\big) \geq 0.
  \end{equation*}
  Note that the condition on $\alpha$ means that the area is
  increasing along the variation.
\end{theorem}
\begin{proof}
  Non-negativity of the Hawking-mass is obvious from
  lemma~\ref{thm:init-integral}. To observe monotonicity, we compute
  the variation of the Hawking-mass. We denote $F(\Sigma,s) =
  \Sigma_s$.
  \begin{equation*}
    (16\pi)^{3/2} \DDeval{}{s}{s=0} m_H
    =
    \frac{1}{2|\Sigma|^{1/2}}\left(\int_\Sigma \alpha H \dmu
    \right)\left(16\pi - \int_\Sigma\dmu\right)
    - |\Sigma|^{1/2} \int_\Sigma \lambda \alpha H \dmu
  \end{equation*}
  as equation~(\ref{eq:1}) implies that the variation of $\int_\Sigma
  H^2\dmu$ is given by $\lambda H$. This yields
  \begin{equation*}
    (16\pi)^{3/2} \DDeval{}{s}{s=0} m_H
    =
    \frac{1}{2|\Sigma|^{1/2}}\left(\int_\Sigma \alpha H \dmu
    \right)\left(16\pi -2\lambda|\Sigma| -\int_\Sigma H^2 \dmu\right).
  \end{equation*}
  Lemma~\ref{thm:init-integral} impies non-negativity of the right
  hand side.
\end{proof}
Subsequently we will assume that the manifold $(M,g)$ is
$(m,\eta,\sigma)$-asymptotically Schwarzschild, and $\Sigma\subset M$
is a surface with $\rmin \geq r_0$ large enough. The particular $r_0$
will only depend on $m$, $\eta$ and $\sigma$, and we will no longer
explicitly denote the dependence on these quantities. Similarly
constants denoted with a capital $C$ are understood to depend on $m$,
$\eta$ and $\sigma$, in addition to quantities explicitly mentioned.
In contrast, constants denoted by $c$ will not have any implicit
dependency. We will no longer require the condition $\ScalM\geq 0$.
It turns out that these surfaces are very round, and have $\int_\Sigma
H^2 \dmu$ very close to $16\pi$.
\begin{lemma}
  \label{thm:initial-roundness}
  Let $(M,g)$ be $(m,\eta,\sigma)$-asymptotically flat. Then there
  exists $r_0= r_0(m,\eta,\sigma)$ and a constant $C =
  C(m,\eta,\sigma)$ such that for all spherical surfaces $\Sigma\subset
  M\setminus B_{r_0}(0)$ satisfying equation~\eqref{eq:1} with
  $\lambda>0$ and $H>0$, we have the following estimates.
  \begin{align*}
    &
    \int_\Sigma|\Acirc|^2 \dmu
    \leq
    C \rmin^{-1}
    \\
    &
    \left| \int_\Sigma H^2\dmu - 16\pi \right|
    \leq 
    C \rmin^{-1}
    \\
    &
    \lambda |\Sigma|
    \leq
    8\pi + C\rmin^{-1}    
  \end{align*}
\end{lemma}
\begin{proof}
  From lemma~\ref{thm:init-integral} we get the bound
  \begin{equation*}
    \int_\Sigma H^2 \dmu
    \leq
    16 \pi - \int_\Sigma \ScalM\dmu
  \end{equation*}
  As $|\ScalM|\leq C(\eta)r^{-4}$ we find that in view of
  lemma~\ref{thm:integral-powers}
  \begin{equation*}
    \int_\Sigma H^2 \dmu
    \leq
    16 \pi + C(m,\eta,\sigma) \rmin^{-2} \int_\Sigma H^2\dmu
  \end{equation*}
  So if $\rmin$ is large enough, eventually
  \begin{equation*}
    \int_\Sigma H^2 \dmu \leq 16\pi + C(m,\eta,\sigma) \rmin^{-2}.
  \end{equation*}
  We can write the Gauss equation (\ref{eq:14}) in the following form
  \begin{equation*}
    \ScalSig
    \leq
    \ScalSig + |\Acirc|^2
    = \half H^2 + \ScalM -2\Ric(\nu,\nu)
  \end{equation*}
  Integrating gives $8\pi$ on the right hand side, and the ambient
  curvature terms can be estimated in view of
  lemma~\ref{thm:integral-powers}. This gives
  \begin{equation*}
    16\pi \leq \int_\Sigma H^2\dmu + C(m,\eta,\Sigma)\rmin^{-1}.
  \end{equation*}
  Going back to the first equation of lemma~\ref{thm:init-integral},
  we see that the $\half\int H^2\dmu$ on the left takes up all of the
  $8\pi$ on the right. We infer
  \begin{equation*}
    \lambda |\Sigma|
    +
    \int_\Sigma |\nabla\log H|^2 + |\Acirc|^2 \dmu
    \leq
    C\rmin^{-1}.
  \end{equation*}
\end{proof}
The initial bound on $\Acirc$ derived above is crucial for higher
curvature estimates on $\Sigma$. We will follow the strategy outlined
in \cite[Section 2]{Kuwert-Schatzle:2001}. Unfortunately the estimates
there were derived in flat ambient space. Thus, although the following
estimate does not differ in major points, we have to repeat the
argument to see the effect of the ambient curvature. We do not have
to consider local estimates, due to the global bound on
$\|\Acirc\|_{L^2{\Sigma}}$ and $\int_\Sigma H^2\dmu$.
\begin{lemma}
  \label{thm:replace-d2H-by-lapH}
  \begin{equation}
    \label{eq:15}
    \int_\Sigma |\nabla^2 H|^2  + \frac{1}{4} H^2 |\nabla H|^2 \dmu
    =
    \int_\Sigma |\Delta H|^2 + \RiemM_{ijik} \nabla_i H \nabla_k H +
    \Acirc_{ik}\Acirc_{jk} \nabla_k H \nabla_j H \dmu
  \end{equation}
\end{lemma}
\begin{proof}
  Compute
  \begin{equation}
    \label{eq:16}
    \begin{split}
      \nabla_i\nabla_i\nabla_j H  - \nabla_j \nabla_i \nabla_i H
       &=
       - \RiemSig_{ijik} \nabla^k H
       \\
       &=
       - \RiemM_{ijik} - A_{ik}A_{ij} + A_{ii} A_{jk}
    \end{split}
  \end{equation}
  Splitting the terms containing $A$ into the trace an traceless part
  gives
  \begin{equation*}
    A_{ii} A_{jk} - A_{ik} A_{ij} = \frac{1}{4} H^2 \gamma_{jk} - \Acirc_{ik}\Acirc_{ij}.
  \end{equation*}
  Substituting into equation (\ref{eq:16}), integration and
  integration by parts yields the claim.
\end{proof}
From the equation (\ref{eq:1}) we find that
\begin{equation*}
  \Delta H = \frac{\lambda}{2} H + H |\Acirc|^2 + H \Ric(\nu,\nu).
\end{equation*}
Squaring and integrating yields
\begin{equation*}
  \int_\Sigma |\Delta H|^2 \dmu
  \leq
  c{\lambda^2} \int_\Sigma H^2\dmu
  +
  c\int_\Sigma H^2|\Acirc|^2 \dmu
  +
  c\int_\Sigma H^2 \RicM(\nu,\nu) \dmu.
\end{equation*}
Recall that lemma~\ref{thm:init-integral} provides a bound on $\int
H^2\dmu$. As $|\Ric|\leq C\rmin^{-3}$ both of the
terms containing $\int_H^2\dmu$ can be estimated. Furthermore for all $\eps>0$
\begin{equation*}
  c \int_\Sigma H^2 |\Acirc|^2 \dmu
  \leq
  \eps \int_\Sigma H^4 |\Acirc|^2 \dmu
  +
  c(\eps) \int_\Sigma |\Acirc|^6 \dmu
\end{equation*}
Thus we arrive at the following estimate.
\begin{lemma}
  \label{thm:estimate-d2HA}
  For all $\eps>0$ we have the estimate
  \begin{equation*}
    \begin{split}
      &\int_\Sigma |\nabla^2 H|^2
      + H^2 |\nabla H|^2 \dmu
      \\
      &\quad
      \leq
      C\rmin^{-6}
      + \rmin^{-2} |\Sigma|^{-2}
      + \eps \int_\Sigma H^4|\Acirc|^2\dmu  
      + c(\eps) \int_\Sigma |\Acirc|^6\dmu.
    \end{split}
  \end{equation*}
\end{lemma}
The next extimate uses Simons identity (\ref{eq:8}) to derive gradient
estimates.
\begin{lemma}
  \label{thm:estimate-d2HB}
  \begin{equation*}
    \begin{split}
      &
      \int_\Sigma |\nabla^2 H|^2 + H^2 |\nabla A|^2 + H^4|\Acirc|^2
      \dmu
      \\
      &\quad
      \leq
      c\rmin^{-2} |\Sigma|^{-2}
      + C\rmin^{-6}
      + C \int_\Sigma |\Acirc|^6 + |\Acirc|^2|\nabla\Acirc|^2\dmu
    \end{split}
  \end{equation*}
\end{lemma}
\begin{proof}
  Multiply Simons identity, equation~(\ref{eq:8}) by $H^2$, integrate
  over $\Sigma$, and do an integration by parts on the left hand side,
  and on the first and the last term on the right hand side of
  equation~(\ref{eq:8}).
  \begin{equation}
    \label{eq:18}
    \begin{split}
      &
      \int_\Sigma
      \nabla_k (H^2 \Acirc^{ij})\nabla_k\Acirc_{ij}
      + \half H^4|\Acirc|^2
      \dmu
      \\
      & \quad
      =
      \int_\Sigma
      H^2\la \div \Acirc, \nabla H\ra
      + 2\la \div \Acirc,\omega\ra
      - |H|^2 |\Acirc|^4
      + H^2 \Acirc*\Acirc*\RiemM \dmu
    \end{split}
  \end{equation}
  As $\div \Acirc = \half \nabla H + \omega$ by the Codazzi
  equation~(\ref{eq:6}), the first term on the right gives
  \begin{equation*}
    \begin{split}
      - \int_\Sigma \la H^2 \Acirc, \nabla H\ra \dmu
      &=
      \int_\Sigma \half H^2 |\nabla H|^2
      + H^2 |\omega|^2
      + H^2 \la \omega, \div \Acirc\ra \dmu
      \\
      &\qquad
      + \int_\Sigma
      2 H \Acirc(\div \Acirc,\div\Acirc)
      + 4H \Acirc(\omega,\div\Acirc) + 2\Acirc(\omega,\omega)
      \dmu
    \end{split}
  \end{equation*}
  After sorting terms and using $\div\Acirc = \half \nabla H + \omega$
  in multiple places, we cast equation~(\ref{eq:18}) into the form
  \begin{equation}
    \label{eq:19}
    \begin{split}
      &
      \int_\Sigma H^2 |\Acirc|^2 + \half H^4|\Acirc|^2 \dmu
      \\
      &\quad
      \leq
      \int_\Sigma
      \half H^2 |\nabla H|^2
      + H^2 |\Acirc|^4 
      + A*A*\omega*\omega
      + H \Acirc*\nabla\Acirc*\nabla\Acirc
      \dmu
      \\
      &\qquad
      +\int_\Sigma      
      H A* \omega*\nabla\Acirc
      + H^2 \Acirc * \Acirc *\RiemM
      \dmu
    \end{split}
  \end{equation}
  We estimate the error terms individually, while keeping in mind the bounds
  from lemma~\ref{thm:initial-roundness}.
  \begin{align*}
    \int_\Sigma H \Acirc * \nabla \Acirc * \nabla \Acirc \dmu
    &\leq
    \eps \int_\Sigma H^2 |\nabla\Acirc|^2 \dmu
    + c(\eps) \int_\Sigma |\Acirc|^2 |\nabla\Acirc|^2\dmu,
    \\
    \int_\Sigma H A * \omega*\nabla \Acirc \dmu
    &\leq
    \eps \int_\Sigma H^2|\nabla \Acirc|^2 \dmu
    + c(\eps) \int_\Sigma |A|^2 |\omega|^2 \dmu,
    \\
    \int_\Sigma A * A * \omega * \omega \dmu
    &\leq
    c \sup_\Sigma |\omega|^2 \int |A|^2\dmu
    \leq C \rmin^{-6},
    \intertext{and}
    \int_\Sigma H^2 |\Acirc|^2 |\RiemM|\dmu
    &\leq
    \eps \int_\Sigma H^4 |\Acirc|^2 \dmu
    + c(\eps) \sup_\Sigma |\RiemM|^2 \int_\Sigma |\Acirc|^2\dmu
    \\
    &\leq
    \eps \int_\Sigma H^4 |\Acirc|^2 \dmu
    + C\rmin^{-7}.
  \end{align*}
  By choosing $\eps = \frac{1}{8}$, and absorbing the terms with the factor
  $\eps$ on the left hand side of equation~(\ref{eq:19}), we infer
  \begin{equation*}
    \int_\Sigma H^2 |\Acirc|^2 + H^4|\Acirc|^2 \dmu
    \leq
    C\rmin^{-6}
    + C \int_\Sigma H^2 |\nabla H^2|
    + |\Acirc|^6
    + |\Acirc|^2 |\nabla\Acirc|^2
    \dmu.
  \end{equation*}
  Combining with the estimate from lemma~\ref{thm:estimate-d2HA} for small
  enough $\eps$ in that lemma, we infer the claimed estimate.
\end{proof}
We want to derive an estimate for $\int|\nabla^2\Acirc|^2\dmu$ from
this estimate.
\begin{lemma}
  \label{thm:replace-d2A0-by-lapA0}
  \begin{equation*}
    \begin{split}
      \int_\Sigma |\nabla^2 \Acirc|^2\dmu
      &
      =
      \int_\Sigma |\Delta \Acirc|^2
      + \RiemM * \nabla\Acirc * \nabla \Acirc
      + \RiemM * \Acirc * \nabla^2 \Acirc
      \dmu
      \\
      & \qquad
      + \int_\Sigma
      A * A * \nabla \Acirc * \nabla \Acirc
      + A * A *\Acirc * \nabla^2 \Acirc
      \dmu
    \end{split}
  \end{equation*}
\end{lemma}
\begin{proof}
  \begin{equation*}    
    \begin{split}
      &\int_\Sigma
      \nabla_i\nabla_j\Acirc_{lm} \nabla_i\nabla_j\Acirc_{lm}
      \dmu
      \\
      &\quad=
      \int_\Sigma
      \nabla_j \nabla_i \Acirc_{lm} \nabla_i\nabla_j\Acirc_{lm}
      + \RiemSig * \nabla \Acirc * \nabla \Acirc
      \dmu
      \\
      &\quad=
      \int_\Sigma
      - \nabla_i \nabla_j \nabla_i \Acirc_{lm} \nabla_i\nabla_j\Acirc_{lm}
      + \RiemSig * \Acirc * \nabla^2 \Acirc
      \dmu
      \\
      &\quad=
      \int_\Sigma
      - \nabla_j \nabla_i \nabla_i \Acirc_{lm} \nabla_i\nabla_j\Acirc_{lm}
      + \RiemSig * \nabla \Acirc * \nabla \Acirc
      + \RiemSig * \Acirc * \nabla^2 \Acirc
      \dmu
      \\
      &\quad=
      \int_\Sigma |\Delta\Acirc|^2 
      + \RiemSig * \nabla \Acirc * \nabla \Acirc
      + \RiemSig * \Acirc * \nabla^2 \Acirc
      \dmu
    \end{split}   
  \end{equation*}
  In view of the Gauss equation, $\RiemSig = \RiemM + A*A$, and the
  claim follows.
\end{proof}
As $\Delta \Acirc$ can be computed using Simons identity, we find the
following estimate.
\begin{lemma}
  \label{thm:estimate-d2A0}
  \begin{equation*}
    \begin{split}
      &\int_\Sigma |\nabla^2 \Acirc|^2
      + H^2|\nabla\Acirc|^2
      + H^4|\Acirc|^2
      \dmu
      \\
      &\quad
      \leq
      C\rmin^{-6}
      + C \rmin^{-2} |\Sigma|^{-2}
      + c \int_\Sigma |\Acirc|^6 + |\Acirc|^2|\nabla \Acirc|^2\dmu
    \end{split}
  \end{equation*}
\end{lemma}
\begin{proof}
  The Simon's identity implies that
  \begin{equation*}
    (\Delta \Acirc)^2
    \leq c (
    |\nabla^2 H|^
    + H^4 |\Acirc|^2
    + |\Acirc|^6
    + |\Acirc|^2 |\RiemM|^2
    + |(\nabla \omega)^0|^2)
  \end{equation*}
  For later reference, we compute $(\nabla\omega)^0$ as follows
  \begin{equation*}
    \begin{split}
      2\nabla_i\omega_j - \div \omega \gamma_{ij}
      &=
      \big(( \nabM \RicM(\nu,\cdot) )^T \big)^0_{ij}
      + 2 \Acirc_{ik}\RicM_{kj} - \la \Acirc, \RicM^T\ra
      \\
      &\phantom{=}
      - 2\Acirc_{ij} \Ric(\nu,\nu)
      + H (\RicM^T)^0_{ij}.
    \end{split}
  \end{equation*}
  Here $(\cdot)^T$ denotes tangential projection in all arguments, and
  $(\cdot)^0$ denotes taking the traceless part. For now, we will
  just use $\nabla \omega = \nabla\RiemM + A*\RiemM$.
  
  Combining the above expression for $|\Delta\Acirc|^2$ with
  lemma~\ref{thm:replace-d2A0-by-lapA0} gives
  \begin{equation*}
    \begin{split}
      \int_\Sigma |\nabla^2\Acirc|^2 \dmu
      &\leq
      c\int_\Sigma
      |\nabla^2 H|^2
      + H^4|\Acirc|^2
      + |\Acirc|^6
      + |A|^2 |\RiemM|^2
      + |\nabM\RiemM|^2
      \dmu
      \\
      & \qquad
      + \int_\Sigma
      \RiemM * \nabla\Acirc * \nabla \Acirc
      + \RiemM * \Acirc * \nabla^2 \Acirc
      \dmu
      \\
      & \qquad
      + \int_\Sigma
      A * A * \nabla \Acirc * \nabla \Acirc
      + A * A *\Acirc * \nabla^2 \Acirc
      \dmu
    \end{split}
  \end{equation*}
  We estimate the individual terms.
  \begin{align*}
    \int_\Sigma A * A * \Acirc *\nabla^2 \Acirc \dmu
    &\leq
    \frac{1}{4} \int_\Sigma |\nabla^2\Acirc|^2\dmu
    + c \int_\Sigma H^4|\Acirc|^2 + |\Acirc|^6 \dmu,
    \\
    \int_\Sigma A*A*\nabla\Acirc*\nabla\Acirc \dmu
    &\leq
    c \int_\Sigma H^2 |\nabla \Acirc|^2
    + |\Acirc|^2|\nabla\Acirc|^2\dmu,
    \\
    \int_\Sigma \RiemM * \Acirc * \nabla^2 \Acirc
    &\leq
    \frac{1}{4} \int_\Sigma |\nabla^2\Acirc|^2\dmu
    + c \int_\Sigma |\Acirc|^2 |\RiemM|^2\dmu,
    \\
    &\leq
    \frac{1}{4} \int_\Sigma |\nabla^2\Acirc|^2\dmu
    + C \rmin^{-7},
    \\
    \int_\Sigma \RiemM * \nabla \Acirc * \nabla \Acirc \dmu
    &\leq
    c \sup_\Sigma |\RiemM| \int_\Sigma |\nabla \Acirc|^2\dmu,
    \\
    \int_\Sigma A * A * \RiemM * \RiemM \dmu
    &\leq
    C\rmin^{-6},
    \intertext{and}
    \int_\Sigma \nabM\RiemM *\nabM \RiemM \dmu
    &\leq
    C\rmin^{-6}.
  \end{align*}
  Absorbing the terms $\int_\Sigma |\nabla^2\Acirc|^2$ appearing on the
  right into the left hand side, we arrive at the estimate
  \begin{equation}
    \label{eq:21}
    \begin{split}
      \int_\Sigma |\nabla^2 \Acirc|^2\dmu
      &\leq
      c\int_\Sigma
      |\nabla^2 H|^2
      + H^2|\nabla\Acirc|^2
      + H^4 |\Acirc|^2
      + |\Acirc|^6
      + |\Acirc|^2|\nabla\Acirc|^2
      \dmu
      \\
      &\quad
      + C\rmin^{-3} \int_\Sigma |\Acirc|^2\dmu
      + C\rmin^{-6}  
    \end{split}
  \end{equation}
  In view of lemma~\ref{thm:estimate-d2HB}, this yields the claim,
  modulo an estimate on $\int_\Sigma |\Acirc|^2\dmu$. We derive this
  estimate from the Simons idendity. To this end integrate
  equation~(\ref{eq:8}). This gives, after integration by parts,
  \begin{equation}
    \label{eq:17}
    \int_\Sigma |\nabla \Acirc|^2 + \half H^2|\Acirc|^2 \dmu
    =
    \int_\Sigma
    \la \div \Acirc, \nabla H\ra
    + 2 \la \div\Acirc, \omega\ra
    + |\Acirc|^4
    + \Acirc * \Acirc * \RiemM
    \dmu
  \end{equation}
  We use $\div \Acirc = \half \nabla H + \omega$ to compute
  \begin{equation*}
    \la \div \Acirc, \nabla H\ra 
    =
    \half |\nabla H|^2 + \la \omega, \nabla H\ra
    =
    \half |\nabla H|^2 + 2 \la \omega, \div \Acirc\ra - 2 |\omega|^2
  \end{equation*}
  Hence,
  \begin{equation*}
    \la \div \Acirc, \nabla H\ra
    + 2 \la \div\Acirc, \omega\ra
    \leq
    \half |\nabla H|^2 + \half |\nabla\Acirc|^2 + c|\omega|^2.    
  \end{equation*}
  In combination with (\ref{eq:17}), we infer
  \begin{equation}
    \label{eq:20}
    \int_\Sigma |\nabla \Acirc|^2 + H^2|\Acirc|^2 \dmu
    \leq
    C\rmin^{-4} + \int_\Sigma |\nabla H|^2 + |\Acirc|^4 \dmu.
  \end{equation}
  Recall that $\Sigma$ satisfies equation~(\ref{eq:1}). Multiplication
  with $\half H$ and integration yields
  \begin{equation*}
    \int_\Sigma |\nabla H|^2 - H^2|\Acirc|^2 = \int_\Sigma
    H^2\RicM(\nu,\nu) + \frac{\lambda}{2} H^2 \dmu.
  \end{equation*}
  In view of lemma~\ref{thm:initial-roundness} this yields
  \begin{equation*}
    \int_\Sigma |\nabla H|^2 - H^2|\Acirc|^2
    \leq
    C\rmin^{-3} + C \rmin^{-1}|\Sigma|^{-1}.
  \end{equation*}
  Plugging this into equation (\ref{eq:20}), we infer
  \begin{equation}
    \label{eq:23}
    \int_\Sigma |\nabla \Acirc|^2 \dmu
    \leq
    C\rmin^{-3} + C \rmin^{-1}|\Sigma|^{-1} + \int_\Sigma |\Acirc|^4\dmu.
  \end{equation}
  The term we wanted to estimate in equation~(\ref{eq:21}), was
  $\rmin^{-3} \int |\nabla\Acirc|^2\dmu$, thus we have to examine the term
  \begin{equation}
    \label{eq:22}
    C\rmin^{-3} \int_\Sigma |\Acirc|^4 \dmu
    \leq
    C\rmin^{-6} \int_\Sigma |\Acirc|^2 \dmu + \int_\Sigma |\Acirc|^6\dmu.
  \end{equation}
  Combining equations~(\ref{eq:22}),~(\ref{eq:23}) and~(\ref{eq:21})
  yields the desired estimate.
\end{proof}
We now need a multiplicative Soboloev-inequality. This is the same as
\cite[Lemma 2.5]{Kuwert-Schatzle:2001}.
\begin{lemma}
  \label{thm:mult-sobolev}
  There exists a constant $C$ such that for all $(M,g)$ which are 
  $(m,\eta,\sigma)$-asymptotically Schwarzschild there exists
  $r_0=r_0(m,\eta,\sigma)$ such that for all $\Sigma\subset M\setminus
  B_{r_0}(0)$ we have
  \begin{equation*}
    \begin{split}
      &\int_\Sigma |\Acirc|^6 + |\Acirc|^2|\nabla\Acirc|^2\dmu
      \\
      &\quad
      \leq
      C \left(\int_\Sigma |\Acirc|^2\dmu\right)
      \left(\int_\Sigma |\nabla^2 A|^2 + |A|^2|\nabla A|^2 + |A|^4
        |\Acirc|^2\dmu \right).
    \end{split}
  \end{equation*}
\end{lemma}
\begin{proof}
  The proof is the same as in \cite[Lemma 2.5]{Kuwert-Schatzle:2001},
  except that we do not have to deal with a cutoff function here.
  However we must use the version of the Michael-Simon-Soboloev
  inequality for asymptoticallf flat manifolds. This is the place from
  where we get the restriction on $r_0$.
\end{proof}
\begin{theorem}
  \label{thm:int-curvature-estimate-1}
  Let $(M,g)$ be $(m,\eta,\sigma)$-asypmtotically Schwarzschild. Then
  there exists $r_0=r_0(m,\eta,\sigma)$ and $C=C(m,\eta\sigma)$ such
  that any surface $\Sigma\subset M\setminus B_{r_0}(0)$ satisfying
  equation~(\ref{eq:1}) with $H>0$ and $\lambda>0$ also satisfies the
  estimates
  \begin{equation*}
    \int_\Sigma |\nabla^2 A|^2 + H^2|\nabla A|^2 +
    H^4|\Acirc|^2 \dmu
    \leq
    C\rmin^{-6} + C \rmin^{-2}|\Sigma|^{-2}.
  \end{equation*}
\end{theorem}
\begin{proof}
  This is a consequence of lemma~\ref{thm:initial-roundness},
  lemma~\ref{thm:estimate-d2A0} and the multiplicative
  Sobolev-inequality in lemma~\ref{thm:mult-sobolev}.

  In addition we used the fact that by the Codazzi equations
  \begin{equation*}
    |\nabla A| \leq c |\nabla \Acirc| + |\omega|
  \end{equation*}
  and
  \begin{equation*}
    |\nabla^2\Acirc| \leq c|\nabla^2 \Acirc| + |\nabla\omega|
  \end{equation*}
\end{proof}
\begin{corollary}
  Let $(M,g)$ and $\Sigma$ be as in
  theorem~\ref{thm:int-curvature-estimate-1}. Then
  \begin{equation*}
    \int_\Sigma |\Acirc|^2 + |\nabla \log H|^2 \dmu
    \leq
    C\rmin^{-2} + \rmin^{-6}|\Sigma|^2
  \end{equation*}
  and
  \begin{equation*}
    \int_\Sigma |\Acirc|^4 \dmu
    \leq
    C\rmin^{-4} + C\rmin^{-2}|\Sigma|^{-1}.
  \end{equation*}
\end{corollary}
\begin{proof}
\end{proof}
  
  
  
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "master"
%%% End: 


==> draft_commands.tex <==
\usepackage{ifthen}

%% Collect Time and Date Info
\makeatletter
\newcommand{\pt@twodigit}[1]{{\pt@tmp=#1\relax\ifnum\pt@tmp<10 0\fi\the\pt@tmp}}
\newcount\pt@hours
\newcount\pt@minutes
\newcount\pt@tmp
\newcommand{\printtime}{%
\pt@hours=\time%
\divide\pt@hours by 60\relax%
\pt@tmp=\pt@hours%
\multiply\pt@tmp by -60\relax%
\pt@minutes=\time%
\advance\pt@minutes by \pt@tmp%
\pt@twodigit\pt@hours:\pt@twodigit\pt@minutes}

%% How to put Info in the margin
\newlength{\mt@MarginWidth}
\newlength{\mt@PageHeight}
\newlength{\mt@ActualWidth}
\newlength{\mt@MaxWidth}
\newlength{\mt@FontSize}
\newlength{\mt@RightSkip}
\newlength{\mt@TextHeight}
\newlength{\mt@OffsetX}
\newlength{\mt@OffsetY}

\usepackage{eso-pic}
\usepackage{type1cm}
\usepackage{graphicx}

\newcommand{\margintext}[1]{
  \ifx\pdfoutput\undefined\write16{WARNING: Margintext
      will only correctly show up in PS - FILE!}
  \fi
  \AddToShipoutPicture{%
    \setlength{\mt@MarginWidth}{\oddsidemargin}%
    \addtolength{\mt@MarginWidth}{1in}%
    \setlength{\mt@PageHeight}{\paperheight}%
    \setlength{\mt@MaxWidth}{.8\mt@MarginWidth}%
    \setlength{\mt@FontSize}{12mm}%
    \setlength{\mt@RightSkip}{3mm}%
    \setlength{\mt@ActualWidth}{15mm}%
    \ifthenelse{\lengthtest{\mt@ActualWidth > \mt@MaxWidth}}%
    {
      \setlength{\mt@FontSize}{.6\mt@MarginWidth}
      \setlength{\mt@RightSkip}{.2\mt@MarginWidth}
      \setlength{\mt@ActualWidth}{.8\mt@MarginWidth}
    }{}
    \setlength{\mt@OffsetX}{\mt@ActualWidth}
    \setlength{\mt@OffsetY}{0mm}
    \setlength{\unitlength}{1pt}%
    \put(\strip@pt\mt@OffsetX,\strip@pt\mt@OffsetY){%
      \rotatebox{90}
        {
          \makebox[\mt@PageHeight][c]
          {\textcolor[gray]{0.75}{\fontfamily{cmss}
              \fontseries{m}
              \fontshape{n}
              \fontsize{\mt@FontSize}{\mt@FontSize}
              \selectfont{#1}}}
        }
      }
    }
}

%% Collect information from Subversion
% If the file svn_version.tex exists, we will read it, in there
% the command \svnVersion is defined. If the file does not exist, we
% print a warning and set \svnVersion to Unknown
\newboolean{draftmargin}
\setboolean{draftmargin}{false}

\IfFileExists{draft_control.tex}{%
\message{Draft control file exists.}%
\input{draft_control.tex}%
}{% 
\message{ WARNING: draft_control.tex not found.}%
\newcommand{\svnVersion}{???}%
}


\ifthenelse{ \boolean{draftmargin} }
        {
                \margintext{Rev: {\svnVersion}\hspace{1em}Built: {\the\year-\pt@twodigit\month-\pt@twodigit\day} {\printtime}}
        }
        {}

\makeatother



==> layout_commands.tex <==
\usepackage{ifthen}
\usepackage{amsmath}
\usepackage{amsthm}

\makeatletter

\newcommand{\titlefamily}{}
\newcommand{\thmfamily}{}
\newcommand{\sectitlefnt}{}
\newcommand{\subsectitlefnt}{}
\newcommand{\ps@footnumber}{}

\newcommand{\authname}[1]{#1}
\newcommand{\authaddress}[1]{#1}

%% Typesetting equations
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\numberwithin{equation}{section}

\newcommand{\fillbox}{\hspace*{\fill}\ensuremath{\Box}}
\renewcommand{\qedsymbol}{\fillbox}

\ifthenelse{\isundefined{\nofancylayout}}
{%
  \renewcommand{\titlefamily}{\sffamily}%
  \renewcommand{\thmfamily}{\sffamily}%
  \renewcommand{\sectitlefnt}{\titlefamily\bfseries\Large}%
  \renewcommand{\subsectitlefnt}{\titlefamily\bfseries}%
  % 
  %% Paper size and margins
  % \usepackage[shiftmargins]{vmargin}
  % \setpapersize{A4}%
  % \setmarginsrb{35mm}{25mm}{30mm}{25mm}{0mm}{0mm}{10mm}{3\baselineskip}%
  %
  \usepackage{calc}
  \usepackage[totalwidth=136mm,totalheight=213mm,vmarginratio=4:5,footskip=3\baselineskip,hcentering]{geometry}
  
  %% Typesetting the titles
  \renewcommand{\section}{\@startsection%
    {section}%
    {1}%
    {0mm}%
    {-\baselineskip}%
    {\baselineskip}%
    {\sectitlefnt}}%
  \renewcommand{\subsection}{\@startsection
    {subsection}%
    {2}%
    {0mm}%
    {-\baselineskip}%
    {0.5\baselineskip}%
    {\subsectitlefnt}}%
  \renewcommand{\ps@footnumber}{%
    \renewcommand{\@oddhead}{}%
    \renewcommand{\@evenhead}{}%
    \renewcommand{\@oddfoot}{\hfill{\thepage}}%
    \renewcommand{\@evenfoot}{{\thepage}\hfill}}

  % 
  %% Typesetting Paragraphs
  \setlength{\parskip}{1ex plus .5ex minus 0ex}
  \setlength{\parindent}{0em}
  % 
  %% Typesetting Theorems
  \newtheoremstyle{my_plain}%
  {\parskip}% above skip
  {\parskip}% below skip
  {\normalfont\itshape}% body font
  {}% indent
  {\normalfont\thmfamily\bfseries}% head font
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  \newtheoremstyle{my_remark}%
  {\parskip}% aboveskip
  {\parskip}% belowskip
  {\normalfont}% bodyfont
  {}% indent
  {\normalfont\thmfamily\bfseries}% headfont
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  {
    \theoremstyle{my_plain}
    \newtheorem{theorem}{Theorem}[section]
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{definition}[theorem]{Definition}
  }
  
  {
    \theoremstyle{my_remark}
    \newtheorem{remark}[theorem]{Remark}
  }

  \renewcommand{\authname}[1]{\titlefamily #1\hspace*{0pt}\\}
  \renewcommand{\authaddress}[1]{\begin{minipage}{.8\linewidth}\centering\titlefamily\footnotesize
      #1\hspace*{0pt}\end{minipage}\\[1ex]}
}{%
  \newtheorem{theorem}{Theorem}[section]%
  \newtheorem{proposition}[theorem]{Proposition}%
  \newtheorem{corollary}[theorem]{Corollary}%
  \newtheorem{lemma}[theorem]{Lemma}%
  \newtheorem{definition}[theorem]{Definition}%
  \theoremstyle{remark}%
  \newtheorem{remark}[theorem]{Remark}%
}

\newenvironment{abst}{\begin{quote}\small\thmfamily\bfseries
    Abstract. \normalfont\small}{\end{quote}}

\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}
\makeatother

